Expert Aggregation for Financial Forecasting

Machine learning algorithms dedicated to financial time series forecasting have gained a lot of interest. But choosing between several algorithms can be challenging, as their estimation accuracy may be unstable over time. Online aggregation of experts combine the forecasts of a finite set of models in a single approach without making any assumption about the models. In this paper, a Bernstein Online Aggregation (BOA) procedure is applied to the construction of long-short strategies built from individual stock return forecasts coming from different machine learning models. The online mixture of experts leads to attractive portfolio performances even in environments characterised by non-stationarity. The aggregation outperforms individual algorithms, offering a higher portfolio Sharpe Ratio, lower shortfall, with a similar turnover. Extensions to expert and aggregation specialisations are also proposed to improve the overall mixture on a family of portfolio evaluation metrics.

==> annexe/annexe-b.tex <==
\section{Variables}
\label{sec:annexb}

\begin{landscape}
\begin{table}{}
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
    Name & Description & Paper & Data base \\
    \hline
    \hline
    mom1m & 1-month momentum & Jegadeesh, Titman 1993 JF & CRSP Monthly \\
    \hline
    mvel1 & Size & Banz 1981 JFE & CRSP Monthly \\
    \hline
    mom12m & 12-month momentum & Jegadeesh 1990 JF & CRSP Monthly \\
    \hline
    chmom & Change in 6-month momentum & Gettleman, Marks 2006 WP & CRSP Monthly \\
    \hline
    maxret & Maximum daily return & Bali, Cakici, Whitelaw 2011 JFE & CRSP Monthly \\
    \hline
    indmom & Industry momentum & Moskowitz, Grinblatt 1999 JF & CRSP Monthly \\
    \hline
    retvol & Return volatility & Ang, Hodrick, Xing, Zhang 2006 JF & CRSP Monthly \\
    \hline
    dolvol & Dollar trading volume & Chordia, Subrahmanyam 2001 JFE & CRSP Monthly \\
    \hline
    sp & Sales to price & Barbee, Mukherji, Raines 1996 FAJ & Compustat Annual \\
    \hline
    turn & Share turnover & Datar, Naik, Radclie 1998 JFM & CRSP Monthly \\
    \hline
    agr & Asset growth & Cooper, Gulen, Schill 2008 JF &
    Compustat Annual \\
    \hline
    nincr & Number of earnings increases & Barth, Elliott, Finn 1999 JAR & Compustat Quarterly \\
    \hline
    rdmve & R\&D to market capitalization & Guo, Lev, Shi 2006, JBFA  & Compustat Annual \\
    \hline
    std\_turn & Volatility of liquidity (share turnover) & Chordia 2001, JFE & CRSP Monthly \\
    \hline
    mom6m & 6-month momentum & Jegadeesh, Titman 1993, JF & CRSP Monthly \\
    \hline
    mom36m & 36-month momentum & Jegadeesh, Titman 1993, JF & CRSP Monthly \\
    \hline
    ep & Earnings to price & Basu 1977, JF & Compustat Annual \\
    \hline
    chcsho & Change in shares outstanding & Ponti, Woodgate 2008, JF & Compustat Annual \\
    \hline
    securedind & Secured debt indicator & Valta 2016, JFQA & Compustat Annual \\
    \hline
    idiovol & Idiosyncratic return volatility & Ali, Hwang, Trombley 2003, JFE & CRSP Monthly \\
    baspread & Bid-ask spread & Amihud Mendelson 1989, JF & CRSP Monthly\\
    \hline
    ill & Illiquidity & Amihud 2002, JFM & CRSP Monthly\\
    \hline
    age & years since first Compustat coverage & Jiang Lee Zhang 2005, RAS & Compustat Annual\\
    \hline
    \end{tabular}
\caption{Variables used}
\label{tab:top_varaibles}
\end{table}
\end{landscape}

% \begin{figure}[h!]
%   \begin{center}
%   \includegraphics[width=\textwidth]{images/Features_ts.png}
%   \end{center}
%   \label{fig:ranksbarplot}
%   \caption{Returns according to each variables/features. Some graph may be rendered unreadable due to huge values.}
% \end{figure}
